Semantic Task Planning for Service Robots in Open World

In this paper, we present a planning system based on semantic reasoning for a general-purpose service robot, which is aimed at behaving more intelligently in domains that contain incomplete information, under-specified goals, and dynamic changes. First, Two kinds of data are generated by Natural Language Processing module from the speech: (i) action frames and their relationships; (ii) the modifier used to indicate some property or characteristic of a variable in the action frame. Next, the goals of the task are generated from these action frames and modifiers. These goals are represented as AI symbols, combining world state and domain knowledge, which are used to generate plans by an Answer Set Programming solver. Finally, the actions of the plan are executed one by one, and continuous sensing grounds useful information, which make the robot to use contingent knowledge to adapt to dynamic changes and faults. For each action in the plan, the planner gets its preconditions and effects from domain knowledge, so during the execution of the task, the environmental changes, especially those conflict with the actions, not only the action being performed, but also the subsequent actions, can be detected and handled as early as possible. A series of case studies are used to evaluate the system and verify its ability to acquire knowledge through dialogue with users, solve problems with the acquired causal knowledge, and plan for complex tasks autonomously in the open world.

==> chapters/__latexindent_temp.tex <==
%!TEX root = ../IEEE.tex

\section{Experiments and Results}\label{section:experiments}

To evaluate the system, we have developed a simulation environment with GAZEBO\footnote{http://gazebosim.org}. The environment contains a domestic house and the model of Kejia. Kejia is equipped with a wheeled mobile base, a single 5-Degree-of-Freedom arm, a 2D laser range finder, an elevator, a pan-tilt, and an RGBD camera. Our system is implemented as nodes in ROS (Robot Operating System). It subscribes all necessary information (arm joint angles, robot pose, recognized objects, etc.) and publishes control messages (navigate to some location, turn on object recognition function to search some object, etc.) which affect the behavior of the robot. The domestic house contains several rooms (bedroom, living room, kitchen, etc.), furniture (bed, table, desk, cupboard, bookshelf, etc.) and some objects (cup, bottle, beer, coke, etc.). For all objects, there are two categories: specific and similar. The specific object has a unique label in the perception system, and this object is bound to this label. Similar objects (apples, same bowl, etc.) share a label in the vision system. For similar objects, their names in the knowledge base are different, the mapping between the vision system and knowledge base depends on location, size, and other properties.

\begin{figure}[ht]
    \centering
    \includegraphics[width=2in]{image/robot.png}
    \caption{The model of Kejia.}
    \label{fig:robot}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.3in]{image/gpsr.png}
    \caption{The domestic environment, which includes two bedrooms, one kitchen, one living room, and one study.}
    \label{fig:env}
\end{figure}

In the experiment, we mainly consider three kinds of uncertainties: HRI uncertainties (vague or erroneous information from users), changing environment (object removed from a known position or object appears in an unexpected place), and execution errors (failed grab, or navigation). The required objects and their positions may be unknown to the robot, so the robot needs to assume that there are objects needed in the place given by the user. Here are five scenarios to show how robots respond to these challenges ({A demo video is available at https://www.youtube.com/watch?v=AE5PDAzkHMw\&t=2s}).

\noindent\textbf{Scenario 1: Jamie requests a coke (vague information).} Initially Jamie and robot were in the living room, the door between the living room and kitchen was unlocked, the robot knew nothing about coke. The robot started by asking Jamie about the location. Jamie offered vague information: in the kitchen. The robot first assumed there was coke in the kitchen table, then started searching in the kitchen by visiting the kitchen table first. On the kitchen table, there was one cup, one water bottle, and one bowl, but no cokes. The robot made the second assumption: the coke was in the cupboard. It visited the cupboard and found two cokes and one beer, then bring one coke to Jamie.\\
\textbf{Scenario 2: Jamie requested a cup from the living table (error information).} Initially Jamie and the robot were in the study, and Jamie asked the robot to go to the living table and brought a cup. The robot first assumed there was a cup in the living table, then started searching by visiting the living table. There was nothing on the living table. The robot abandoned the information from Jamie, it had got the information that a cup was on the kitchen table in Scenario 1. It visited the kitchen table and found one cup, one water bottle, and one bowl, then bring the cup to Jamie.\\
\textbf{Scenario 3: Alice requested a coke (disappearing target).} Initially, Alice and the robot were in the bedroom, the robot knew there was one coke in the cupboard, it visited the cupboard, and started to search the coke, but did not found any coke. The robot removed the item in the knowledge base and made an assumption: there was coke on the kitchen table. However, after it reached the kitchen table, it found no coke on the kitchen table. Then it made another assumption: the coke was on the dining table. The robot navigated to the dining table and found two cokes, finally it taken a coke from the dining table and handed it over to Alice.
\\
\textbf{Scenario 4: Jamie requested a coke and a beer (unexpected target).} Initially, Jamie and the robot were in the study, the robot knew there was one coke in the dining table and a beer in the cupboard, it visited the dining table, and started to search the coke, then it found coke and a beer. An unexpected target (the beer) was found, the robot added a new item to the knowledge base and triggered to replan, a better solution was generated. The robot brought the coke from the dining table to Jamie and then navigated to the dining table, take the beer from the dining table to Jamie.
\\
\textbf{Scenario 5: Jamie requested a bowl (failed grab).} Initially Jamie and the robot were in the living room, the robot known there was one bowl in the kitchen table. It visited the kitchen table and started to search the bowl, then it found the bowl. While when the robot picked up the bowl from the kitchen table, the bowl slipped out of the gripper and fell to the ground. The robot couldn't pick it up from the ground, so it navigated to Jamie and reported this failure.

The demonstration of the robot shows that the system can serve under uncertainties and changing environment by involving assumptions and changing detection. By identifying assumptions or detections that are inconsistent with the knowledge base or not, the robot performs the original plan or makes new assumptions, or replans.


\section{Conclusion}\label{section:conclusion}
In this paper, we present a planning system for a general-purpose service robot, by leveraging HRI, assumptions and continuous sensing, which is aimed at behaving more intelligently in domains that contain incomplete information, under-specified goals, and dynamic changes. Experiments show the robustness of the service robot in the domestic environment. By combining assumption and symbolic planning, the robot can serve without knowing the position of the required object. Proper use of assumptions combined with continuous sensing can be helpful to handle unpredictable domain changes and behavior robust in the open world. In the future, we will address how to make better assumptions to improve planning efficiency.

==> chapters/acknowledgment.tex <==
%!TEX root = ../IEEE.tex

\section*{Acknowledgment}

The authors would like to thank...
